Remove, Reduce, Inform: What Actions do People Want Social Media Platforms to Take on Potentially Misleading Content?

To reduce the spread of misinformation, social media platforms may take enforcement actions against offending content, such as adding informational warning labels, reducing distribution, or removing content entirely. However, both their actions and their inactions have been controversial and plagued by allegations of partisan bias. When it comes to specific content items, surprisingly little is known about what ordinary people want the platforms to do. We provide empirical evidence about a politically balanced panel of lay raters' preferences for three potential platform actions on 368 news articles. Our results confirm that on many articles there is a lack of consensus on which actions to take. We find a clear hierarchy of perceived severity of actions with a majority of raters wanting informational labels on the most articles and removal on the fewest. There was no partisan difference in terms of how many articles deserve platform actions but conservatives did prefer somewhat more action on content from liberal sources, and vice versa. We also find that judgments about two holistic properties, misleadingness and harm, could serve as an effective proxy to determine what actions would be approved by a majority of raters.

==> _archived__background.tex <==

% \section{Background}

% \subsection{How platforms moderate misinformation?}

% In 2018, when Facebook released their moderation guidelines \cite{zuckerbergBlueprintContentGovernance2018}, the report stated that ``these guidelines are designed to reduce subjectivity and ensure that decisions made by reviewers are as consistent as possible'' \cite{zuckerbergBlueprintContentGovernance2018}. The emphasis on reducing subjectivity is not unique to Facebook, but is a trend common across most social media platforms, and oftentimes, their guidelines\footnote{for a more detailed discussion on how platforms' guidelines are structured, see \cite{gillespieCustodiansInternetPlatforms2018}} are strikingly similar. Specific to moderation misinformation, platforms have partnered with independent fact-checking organizations to objectively verify the various facts present in a content \cite{anannyPartnershipPressLessons2018}. However, their guidelines also emphasize on the author's intent and the potential to cause harm as crucial to deciding the course of action against misinformation \cite{vijayaUpdateOurContinuity2020, zuckerbergPreparingElections2018}. While these criteria are important for providing room for unintentional mistakes or even satirical content, their inclusion can make the guidelines appear vague. For instance, Twitter's policy on handling misinformation\footnote{https://help.twitter.com/en/rules-and-policies/manipulated-media} restricts content that is ``significantly altered'' with a ``deliberate intent to mislead'' and is ``likely to cause serious harm''. The vagueness can further result in apparent inconsistencies, or worse, allegations of partisan bias. 
% A recent report found that many of the posts identified as false by prominent fact-checking organisations continued to remain up on various platforms \cite{brennenTypesSourcesClaims}. At the same time, some of the right-wing media have argued that conservative sources are overly censored by platforms \cite{borelFactCheckingWonUs2017}. 

% Furthermore, researchers have argued that platforms' moderation policies are based on their own priorities and incentives \cite{commonFearReaperHow2020,gillespieCustodiansInternetPlatforms2018,paterCharacterizationsOnlineHarassment2016}, including but not limited to the performance of automated tools and efficiency trade-offs \cite{commonFearReaperHow2020}. And despite their emphasis on these guidelines, platforms arbitrarily control many other aspects of the process, from deciding what content is reviewed to how independent reviews are aggregated and then acted upon \cite{gillespieCustodiansInternetPlatforms2018, anannyPartnershipPressLessons2018}. As part of it's first report, Facebook's Data Transparency Advisory Group (DTAG) took note of this and emphasized on a more bottom-up approach to moderation where platform users have an important role to play \cite{bradfordReportFacebookData2019}.

% \subsection{User involvement in moderating online misinformation}
% More recently, platforms such as Twitter and Facebook have launched initiatives toward engaging users in tackling online misinformation \cite{silvermanHelpingFactCheckersIdentify2019,colemanIntroducingBirdwatchCommunitybased2021}. Both initiatives allow users to flag certain content as misinformation, while also sharing additional context and notes. Under Facebook's initiative, user contributions will directly support the work of fact-checkers \cite{silvermanHelpingFactCheckersIdentify2019}, while Twitter will allow these contributions to be accessed by the general public as well \cite{colemanIntroducingBirdwatchCommunitybased2021}.

% In terms of research efforts, prior works suggest that aggregating crowd judgments on the credibility or misleadingness of an article can be used to approximate the expert, i.e., journalists' judgments \cite{, bhuiyanInvestigatingDifferencesCrowdsourced2020}. Resnick et al. [under review] further show that these judgments are more reliable when users are asked to provide a corroborating evidence in support their judgment. Rather than evaluating individual articles, Pennycook and Rand \cite{pennycookFightingMisinformationSocial2019a} focus on evaluating news source quality, and find that lay user judgments can provide a reliable indicator about the quality of the news source. A host of other systems have been proposed that utilize crowdsourcing to scale-up the fact checking process on individual articles \cite{pintoFactCheckingCrowdsourcing2019,kimLeveragingCrowdDetect2018,kimLeveragingVolunteerFact2020}. These systems either allow users to work in close proximity with the experts \cite{pintoFactCheckingCrowdsourcing2019} or rely on their existing activities (flagging content, responding with verified claims, etc.) \cite{kimLeveragingCrowdDetect2018,kimLeveragingVolunteerFact2020} to identify and curb the spread of misinformation. While both platforms' initiatives and prior research have taken major steps toward involving users in fighting misinformation, their focus is limited to the evaluation of content at some level. None of the works emphasize on users' preferences for action against misinformation or make it clear on how these evaluations can provide users' action preferences.

% \subsection{Other challenges with moderating online misinformation}
% Beyond the platforms' guidelines on moderating misinformation, a major challenge concerns with defining misinformation in the first place. Researchers \cite{jrDefiningFakeNews2018,jackLexiconLiesTerms2017} and legal scholars \cite{kleinFakeNewsLegal2017} have argued that a definition based on facts or authenticity may not suffice, as it does not differentiate between satire, unintentional mistakes, and intentionally fabricated content \cite{caplanDeadReckoningNavigating2018}. Even though misinformation is still defined as ``false information that can be verified as such'' \cite{shuFakeNewsDetection2017}, alternate frameworks have proposed a typology that differentiates between misinformation, disinformation, satire, propaganda, etc. \cite{jrDefiningFakeNews2018,jackLexiconLiesTerms2017}. Once again, an important aspect of these frameworks is their emphasis on the intention to mislead and the likelihood of causing harm. These factors, while in the right place, are open to interpretation, and it may not be possible to know their true state. For instance, as platforms have drawn a fixed line between satire and propaganda, many propaganda outlets are trying to avoid action by adding disclaimers about ``satire'' or ``parody'' on their websites, even though their articles can still mislead many users \cite{caplanDeadReckoningNavigating2018}. 

% Focusing on fact-checking, some of the right-wing media have critiqued fact-checking organizations \cite{caplanDeadReckoningNavigating2018} and raised allegations of partisan bias (i.e., pro-liberal). This has led to a general lack of distrust among certain users \cite{brandtzaegHowJournalistsSocial2017}. Furthermore, when it comes to ongoing scientific discoveries, for instance, the origin of COVID-19 pandemic, ``facts'' can be fluid, and what is considered accurate today may turn out to be false later on \cite{bakerChallengesRespondingMisinformation2020}. 

% Some researchers \cite{zhangStructuredResponseMisinformation2018a} have also focused on identifying a set of indicators that signify the credibility of a content, as a way to identify and analyse misinformation. However, their proof-of-concept found that independent annotations by a crowd on these indicators were not always correlated, suggesting that the indicators may be interpreted differently. Further work in this 
% direction also pointed toward a need for redesigning the annotation task in a way that leads to higher correlation among raters \cite{bhuiyanInvestigatingDifferencesCrowdsourced2020}. We want to emphasize that efforts toward trust and verification of content have an important role to play when it comes to establishing the truth \cite{caplanDeadReckoningNavigating2018}, making users more informed, or setting credibility standards \cite{zhangStructuredResponseMisinformation2018a}. However, simply knowing whether something is true or not does not adequately inform moderation decisions.

% Yet, even if fact-checking organizations can objectively evaluate the ``alterations'' in a content, the uncertainty about the intentions and the likelihood of harm adds a lot of nuance to how the policy gets implemented. 



% Yet, content moderation is inherently subjective, as Gillespie notes in his book, content moderation is about drawing the line between the appropriate and the illicit, and the line may be drawn differently in different cultures and contexts \cite{gillespieCustodiansInternetPlatforms2018}. 

% In other words, the main outcome of content moderation is inherently subjective, yet the platforms are trying to push it toward objectivity. Specifically, the moderation guidelines have been drafted in a way that appropriateness of a content can be determined based on a series of objective characteristics of that content. 

% while a considerable amount of work has been done to highlight the subjectivity involved in content moderation, and the various harm being caused by platform's current approach, it is worth spending some effort to understand how exactly the platforms’ current approach fails to account for that subjectivity and how we use that understanding to inform our evaluation process….

% First and foremost, while content moderation is fundamentally about taking action, platforms have broken it down into a series of objective evaluation of the nature of the content. Let us consider an example...

% To expand on that argument, let us look at some of the platforms' existing guidelines\footnote{for a more detailed discussion on how platforms' guidelines are structured, see \cite{gillespieCustodiansInternetPlatforms2018}}, starting with Facebook's guidelines for determining sexually explicit content\footnote{https://www.facebook.com/communitystandards/adult\_nudity\_sexual\_activity}. The guidelines determine the appropriateness of a content through its objective characteristics such as, the presence of real nude adults (as opposed to fictional or portrayals of art), visible genitalia, and sexual activities like squeezing female breasts. Exceptions are drawn for birth-giving, breastfeeding, and health-related context. Furthermore, the guidelines need to be updated regularly to handle the fluid nature of an offence and the continuously evolving human behavior \cite{gillespieCustodiansInternetPlatforms2018}. As the guidelines evolve to capture new forms of violations or limit unintended overreach, they end up becoming too specific or too vague. For instance, the guidelines referred above were updated in November 2020 to explicitly define breast squeezing as a ``grabbing motion with curved fingers that shows both marks and clear shape change of the breast''\footnote{https://www.facebook.com/communitystandards/recentupdates/adult\_nudity\_sexual\_activity}. And once again, breastfeeding had to be spelled out as an exception to the act. 

% As a counter example, Twitter's policy on handling misinformation\footnote{https://help.twitter.com/en/rules-and-policies/manipulated-media} restricts content that is ``significantly altered'' with a ``deliberate intent'' to mislead and is ``likely'' to cause serious harm. It it likely that the emphasis on significant alteration and a deliberate intent is to provide some room for unintentional mistakes or even satirical content. Yet, even if fact-checking organizations can objectively evaluate the ``alterations'' in a content, the uncertainty about the intentions and the likelihood of harm adds a lot of nuance to how the policy gets implemented. 

% as highlighted by the ``Terror of War'' photograph \footnote{https://time.com/4485344/napalm-girl-war-photo-facebook/}, which depicts child nudity but is nevertheless worth preserving for historical reasons. 

% The limited ability to handle the nuanced cases represents only one side of the criticism these guidelines have drawn. Sarah Roberts, one of the first researchers who studied ``commercial content moderation'' called the guidelines insensitive and oblivious to the harm they cause \cite{robertsCommercialContentModeration2016}. Researchers have also argued that these policies are based on the priorities and incentives of the platforms \cite{commonFearReaperHow2020,gillespieCustodiansInternetPlatforms2018,paterCharacterizationsOnlineHarassment2016}, including but not limited to the performance of automated tools and efficiency trade-offs \cite{commonFearReaperHow2020}. Furthermore, despite their emphasis on the guidelines, platforms arbitrarily control many other aspects of the process, from deciding what content is reviewed to how independent reviews are aggregated and then acted upon \cite{gillespieCustodiansInternetPlatforms2018, anannyPartnershipPressLessons2018}. All this can lead to apparent inconsistencies in the way these guidelines are formulated \cite{paterCharacterizationsOnlineHarassment2016} and enacted \cite{commonFearReaperHow2020}. Facebook's Data Transparency Advisory Group further took note of this and emphasized on a more bottom-up approach to moderation where platform users have an important role to play \cite{bradfordReportFacebookData2019}.

% \textbf{Our approach:} The arguments from above suggest that - i) the moderation pipeline when carried out as a series of (somewhat) objective evaluations of the content has limited ability to accommodate the many nuances of moderation, and ii) platform users need to play a more important role in the moderation pipeline. Inspired by these arguments, we explore how users can be involved in the moderation pipeline beyond just carrying out an objective evaluation of the content. And since moderation is fundamentally about deciding the course of action against a content, we focus on the obvious choice of directly collecting users' preferences for action against a content, and further use that as a metric to evaluate the decisions that platforms can take. Additionally, it may also be possible to explicitly emphasize on a subjective evaluation of the content by the users. For e.g., evaluating the content for nudity can be largely objective, but evaluating it for pornography may involve subjective considerations such as, the aim of the poster, the effect on the viewer, aesthetic judgment, etc. (see Gillespie \cite{gillespieCustodiansInternetPlatforms2018}). In case of misinformation, we ask users to provide their subjective judgments about how misleading and harmful the content is, which goes beyond a fixed set of objective characteristics about the content such as, its factual claims, accuracy of the headline, the properties of the sources, etc. \cite{zhangStructuredResponseMisinformation2018a}. 

% Finally, one more criticism related to close ended responses, but we do not address that because it has some benefits

% iii) A final way in which platforms try to objectify the moderation process is by requiring close-ended reviews rather than open-ended reviews. A close-ended review may constitute a binary response to questions such as ``is this objectionable'', or the content's categorization as per an existing classification schema. This approach is particularly evident in the flagging mechanisms adopted by different platforms which allows users to report potentially problematic content for further review \cite{gillespie_custodians_2018}. The mechanism is often designed in a way that streamlines the platforms' moderation process but only provides a ``thin form of expression'' \cite{gillespie_custodians_2018} to the users. The close-ended forms leave little room for the users to appropriately contextualize their complaint or express the degree and reasons for their concern. Prior research has also found that the mechanism may fail to protect minority user groups \cite{duguay_queer_2020} as well as invalidate the experience of certain users when it does not fit into their existing schema \cite{blackwell_classification_2017}. 

% Despite these limitations, close-ended responses do serve an important purpose. In the most straightforward cases, they reduce the cost and effort associated with the process -- it is easier for the users to provide a binary response or choose a category, and it is easier for the platforms to arrive at the decision by analytically summarizing these responses.
% In summary, the same can be said for all moderation policies -- they serve an important purpose, but nevertheless leave a gap -- the \emph{moderation gap} -- especially as it concerns with the outcome of moderation. And whether they want it or not, platforms end up bridging this gap while enforcing their policies.

% A different approach to moderating misinformation is through government regulations. In the US, Section 230 gives platforms the right but not the responsibility to remove problematic content which is not classified as unlawful by any other provision of the law \cite{gillespie_custodians_2018}. Contrary to that, lawmakers in Germany have recently passed a legislation (NetzDG\footnote{https://en.wikipedia.org/wiki/Network\_Enforcement\_Act}) to fine social media companies and search engines for misleading content that engages in hate speech. However, the legislation inadvertently puts even more power into the hands of the platforms to adjudicate the moderation decisions \cite{caplan_dead_2018}, rather than acknowledging the gap that already exists or pushing platforms to systematically address this gap.

% Pinto et al. \cite{pinto_towards_2019} proposed another system that utilizes crowdsourcing to scale-up the fact checking of individual content. Specifically, any user can propose a verification or rebuttal of a content which can then be voted upon by other users. And in cases of disagreement within the crowd, experts (for instance, journalists) can be sought to review and update the proposal. While promising in theory, their work lacks any empirical evidence to demonstrate the effectiveness of this design. As an alternative approach, researchers have looked at utilizing users' existing activities -- such as, flagging a content as misinformation \cite{kim_leveraging_2018} or responding to a content with verified claims \cite{kim_leveraging_2020} -- as a way to identify emerging instances of misinformation. The algorithm by Kim et al. \cite{kim_leveraging_2018} can be particularly useful in streamlining the fact-checking process by prioritizing which stories need to be fact-checked first. 







==> _archived__results.tex <==
\section{Results}

\label{sec:results}

\subsection{Hierarchy of Severity}

\textbf{RQ\ref{rq-hierarchy}: Is there a hierarchy of perceived severity of actions among informed lay raters?}

Table~\ref{tab:overall-descriptives} provides descriptive statistics about the overall frequency with which each of the actions was preferred, aggregating ratings across all articles. The inform action was preferred more often than the reduce action, by both liberal and conservative raters. 

Figure \ref{fig:rq1} shows the Venn diagram of the article sets where a majority of raters preferred each action. For all articles where a majority wanted the reduce action, a majority also wanted the inform action. This suggests that the raters perceive a hierarchy of severity between different actions, where \textit{inform} is considered the least severe, followed by \textit{reduce}, and then \textit{remove}. 

Additionally, the presentation order (i.e., the order in which inform and reduce actions were presented to the raters) did have some impact on their ratings. Comparing between column 2 and 3 of Table ~\ref{tab:presentation-order}, we see that presenting \textit{reduce} before \textit{inform} increased the frequency of reduce action -- 28.99\% compared to 25.35\% when \textit{inform} was presented before \textit{reduce}. However, inform was still the most frequently preferred action in both conditions. Furthermore, the Venn diagram of the article sets remained the same for the two conditions, i.e, whenever the majority wanted a reduce action, they also wanted an inform action, irrespective of which action was presented first. 


\begin{table}[t]
% \resizebox{0.7\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
       & All raters & Liberals & Conservatives \\ \hline
Inform & 34.09      & 37.01     & 35.50       \\ \hline
Reduce & 27.17      & 30.06    & 27.40        \\ \hline
Remove & 11.85      & 13.98   & 11.61        \\ \hline
\end{tabular}
% }
\caption{Breakdown by ideology in fraction of ratings where each action was preferred, aggregated across all articles.}
\label{tab:overall-descriptives}
\end{table}

\begin{figure}[t]

  \centering
  \includegraphics[width=0.3\textwidth]{figures/rq1v2.png}
  \caption{Venn diagram of article sets where majority preferred each action.}%
  \label{fig:rq1}
\end{figure}

\begin{table}[t]
% \resizebox{0.7\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
       & All raters & Inform first & Reduce first \\ \hline
Inform & 34.09      & 34.42     & 33.80       \\ \hline
Reduce & 27.17      & 25.35    & 28.99        \\ \hline
Remove & 11.85      & 11.10   & 12.60        \\ \hline
\end{tabular}
% }
\caption{Breakdown by presentation order in fraction of ratings where each action was preferred, aggregated across all articles.}
\label{tab:presentation-order}
\end{table}

\subsection{(Lack of) Consensus on Preferred Actions}
\textbf{RQ\ref{rq-agreement}: How much agreement is there, among informed lay raters, about the preferred actions to be taken on potentially misleading articles?}

Figure~\ref{fig:dist-of-prefs} shows histograms of aggregate action preferences across all 368 articles. For inform action, 62 articles were present in the middle region of the histogram (i.e., where 40-60\% of the raters wanted the action), indicating high disagreement between raters on these articles. If we expanded the middle range to 30-70\%, the number of articles increased to 146. Similar patterns were observed for reduce action as well. 

When the remove action was preferred by a majority, it was almost always a slim majority, with only one article achieving a supermajority of more than 70\% raters. Generally, for all three action types, among articles where more than 50\% raters preferred the action (i.e., the right half of the histograms), it was more common to have 50-70\% of raters prefer the action than to have near universal agreement of 80-100\%. 

Table~\ref{tab:mean-disapproval} summarizes the mean level of disagreement with the majority preference. Averaging across articles, $23.57\%$ disagreed with the majority preference about whether to take an inform action. The mean level of disagreement was lower for the remove action because there were many articles that almost everyone agreed should not be removed. Note that the mean disagreement would only be marginally higher (11.85\% instead of 11.05\%) with a default decision of not removing any article, because even when remove action was preferred by a majority, it was usually a slim majority (also noted above). 



\begin{figure}[bt]
% \figbox{%
  \centering
  \includegraphics[width=1\textwidth]{figures/rq2-partial.png}
% }
% {%
  \caption{Distribution of raters' aggregate preferences for each action type}%
  \label{fig:dist-of-prefs}
% }
\end{figure}

\begin{table}[t]
% \resizebox{0.7\textwidth}{!}{%
\begin{tabular}{|l|l|}
\hline
    %   & All raters & Liberals & Conservatives \\ \hline
Inform & 23.57       \\ \hline
Reduce & 21.12         \\ \hline
Remove & 11.05        \\ \hline
\end{tabular}
% }
\caption{Mean across articles, of percentage of raters who disagreed with the majority preference.}
\label{tab:mean-disapproval}
\end{table}

% \begin{table}[t]
% % \resizebox{0.7\textwidth}{!}{%
% \begin{tabular}{|l|l|l|l|}
% \hline
%       & All raters & Liberals & Conservatives \\ \hline
% Inform & 23.57     & 20.29    & 23.65       \\ \hline
% Reduce & 21.12     & 18.66   & 22.03        \\ \hline
% Remove & 11.05     & 10.17   & 12.66       \\ \hline
% \end{tabular}
% % }
% \caption{Mean level of disagreement, across items, with the majority rating for the item.}
% \label{tab:mean-disapproval}
% \end{table}


\subsection{Partisan Differences in Preferences}


\textbf{RQ\ref{rq-agreement-ideology}: Is there more or less agreement among conservative raters than among liberal raters about their preferred \rev{social media} platform actions?}

Table \ref{tab:reg-agreement} shows the regression coefficients from our model. Except for the inform action, there were no significant differences between conservatives and liberals in their level of agreement with the majority-preference of their respective groups. For inform, conservatives were significantly less likely to agree with the majority-preference of their group, compared to liberals. 


\begin{table}[!htbp] \centering 
 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
 & Inform preference & Reduce preference & Remove preference \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 conservative & $-$0.267$^{***}$ & $-$0.149 & 0.072 \\ 
  & (0.085) & (0.088) & (0.153) \\ 
  & & & \\ 
 Intercept & 1.685$^{***}$ & 1.816$^{***}$ & 3.133$^{***}$ \\ 
  & (0.071) & (0.078) & (0.133) \\ 
  & & & \\ 
\hline \\[-1.8ex] 
Random effects &  &  &  \\ 
sd(rater\_id) & 0.493 & 0.508 & 0.952 \\ 
sd(article\_id) & 0.800 & 0.968 & 1.487 \\ 
Observations & 13,004 & 13,004 & 13,004 \\ 
Log Likelihood & $-$6,374.042 & $-$5,945.140 & $-$3,548.398 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 

 \caption{Regression models for estimating the impact of rater ideology on agreement with the majority preference of their ideology (RQ\ref{rq-agreement-ideology})} 
  \label{tab:reg-agreement} 
  
\end{table} 



\begin{table}[!htbp] \centering 
%   \caption{} 
%   \label{} 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} \\
 & Inform preference & Reduce preference & Remove preference \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 conservative & 0.293 & 0.161 & $-$0.069 \\ 
  & (0.169) & (0.175) & (0.248) \\ 
  & & & \\ 
 source\_pro\_conservative & 1.238$^{***}$ & 1.265$^{***}$ & 1.040$^{***}$ \\ 
  & (0.248) & (0.247) & (0.291) \\ 
  & & & \\ 
 source\_pro\_liberal & 0.113 & 0.188 & $-$0.407 \\ 
  & (0.319) & (0.318) & (0.391) \\ 
  & & & \\ 
 source\_unknown & 0.828$^{**}$ & 0.847$^{**}$ & 0.824$^{**}$ \\ 
  & (0.335) & (0.332) & (0.384) \\ 
  & & & \\ 
 conservative : source\_pro\_conservative & $-$1.052$^{***}$ & $-$1.000$^{***}$ & $-$0.760$^{***}$ \\ 
  & (0.118) & (0.124) & (0.175) \\ 
  & & & \\ 
 conservative : source\_pro\_liberal & 0.763$^{***}$ & 0.658$^{***}$ & 0.907$^{***}$ \\ 
  & (0.146) & (0.156) & (0.249) \\ 
  & & & \\ 
 conservative : source\_unknown & $-$0.540$^{***}$ & $-$0.563$^{***}$ & $-$0.215 \\ 
  & (0.160) & (0.164) & (0.219) \\ 
  & & & \\ 
 Intercept & $-$1.769$^{***}$ & $-$2.258$^{***}$ & $-$4.115$^{***}$ \\ 
  & (0.197) & (0.198) & (0.259) \\ 
  & & & \\ 
\hline \\[-1.8ex] 
Random effects &  &  &  \\ 
sd(Rater\_id) & 1.11 & 1.12 & 1.54 \\ 
sd(article\_id) & 1.88 & 1.84 & 1.97 \\ 
Observations & 13,004 & 13,004 & 13,004 \\ 
Log Likelihood & $-$5,936.760 & $-$5,501.412 & $-$3,244.302 \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{3}{r}{$^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular}

 \caption{Regression Models for estimating the impact of rater ideology and the ideological leaning of the source on rater action preference (RQ\ref{rq-ideology-amount} and RQ\ref{rq-ideology-items}). In all models, `liberal' and `no known bias' are the reference categories.} 
  \label{tab:reg-source-pref} 
  
\end{table} 

\begin{table}[]
\begin{tabular}{|c|c|c|c|c|}
\hline
                  & Estimate & SE    & z.ratio & p-value \\ \hline
Inform preference & -0.122   & 0.178 & -0.684  & 0.4939  \\ \hline
Reduce preference & -0.291   & 0.184 & -1.585  & 0.1130  \\ \hline
Remove preference & -0.103   & 0.269 & -0.384  & 0.7009  \\ \hline
\end{tabular}

\caption{Reporting the contrast on rater ideology (between conservatives and liberals) averaged across all source ideology levels}
\label{tab:contrasts}
\end{table}

\begin{table}[]
    \begin{tabular}{|l|l|l|l|}
    \hline
          & All raters & Only liberals & Only Conservatives \\ \hline
    Inform & 104        & 118           & 108                \\ \hline
    Reduce & 70         & 80            & 74                 \\ \hline
    Remove & 12        & 15            & 22                 \\ \hline
    \end{tabular}
  \caption{No. of articles recommended for each action type based on the aggregate preferences of different user groups}%
  \label{tab:rq1}
\end{table}


\textbf{RQ\ref{rq-ideology-amount}: Do conservative raters prefer that \rev{social media} platforms act on \textit{fewer articles} than liberal raters or vice versa?}

Table \ref{tab:contrasts} shows that, following a marginal means analysis to get an average effect across all source ideology labels, there were no significant differences between conservatives and liberals in terms of how many articles they thought action was appropriate for, and that holds for all actions. 

Table~\ref{tab:rq1} summarizes the majority preferences. There were minor differences in the number of articles that majorities of liberals and conservatives would like to see \rev{social media} platforms act on, as shown in the second and third columns. However, the regression analysis suggests that none of these differences were statistically significant.


\textbf{RQ\ref{rq-ideology-items}: Do conservative raters prefer action on articles from \emph{different sources} than liberal raters?}

% Table \ref{tab:rq1} shows the level of disapproval among conservative and liberal users separately. The pattern suggests that the level of disapproval among conservative users is consistently higher than the level among liberal users. This disparity can be attributed to the distribution of action preferences of each user group (Figure \ref{fig:rq4}). 

Looking at the interaction terms in the same regression model (Table \ref{tab:reg-source-pref}) answers RQ\ref{rq-ideology-items}. The coefficients show the difference from a reference of a liberal rater and a news source labeled as having no known biases. 
Compared to liberal raters, conservatives were significantly less likely to prefer action on articles from pro-conservative sources (see conservative :source\_pro\_conservative in Table \ref{tab:reg-source-pref}). Conversely, on articles from pro-liberal sources, conservative raters were significantly more likely than liberal raters to prefer an action. The results hold for all action types. Conservatives were also less likely to prefer inform and reduce actions on articles from sources whose ideological leaning is not available on MBFC\footnote{https://mediabiasfactcheck.com}.

Table \ref{tab:rq4} shows the differences in terms that may be easier to interpret. While conservative and liberal action preferences were largely correlated on unbiased sources, the correlation dropped quite a bit for sources that are ideologically biased toward either side. We note, however, that positive correlations in the range of 0.55 to 0.80 are still fairly high. 


\begin{table}[]
\begin{tabular}{|l|l|l|l|}
\hline
       & Unbiased source & Pro-liberal source & Pro-conservative source \\ \hline
Inform & 0.92            & 0.66               & 0.79                    \\ \hline
Reduce & 0.91            & 0.68               & 0.80                    \\ \hline
Remove & 0.91            & 0.55               & 0.64                    \\ \hline
\end{tabular}
\caption{Correlations between percentages of conservatives and liberals who preferred an action, on articles from different types of sources.}
\label{tab:rq4}
\end{table}



\subsection{Reducibility to Misleading and Harm Judgments}

\textbf{RQ\ref{rq-proxy}: How well can aggregate judgments of whether an article is misleading and/or harmful predict aggregate preferences for the inform, reduce, and remove actions?}

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{figures/reg-eq.png}
    \caption{Visualizing the decision boundaries in terms of misleading and harm judgments for each action type}
    \label{fig:rq3:reg_eq}
\end{figure}

\begin{table}[!htbp] 
\centering 
\begin{tabular}{@{\extracolsep{5pt}}lccc}  \\[-1.8ex] \hline  \hline  \\[-1.8ex]  \\[-1.8ex] &  \multicolumn{1}{c}{Inform preference} &  \multicolumn{1}{c}{Reduce preference} &  \multicolumn{1}{c}{Remove preference}    \\   \\[-1.8ex] & (1) & (2) & (3)   \\  \hline   \\[-1.8ex]  Misleading judgment & 1.384$^{***}$ & 1.089$^{***}$ & 0.728$^{***}$   \\   & (0.055) & (0.055) & (0.021)   \\  Harm judgment & 0.803$^{***}$ & 0.682$^{***}$ & 0.236$^{***}$   \\   & (0.057) & (0.062) & (0.034)   \\  Misleading:Harm & -0.169$^{***}$ & -0.104$^{***}$ &   \\   & (0.015) & (0.015) &   \\  Intercept & -5.575$^{***}$ & -5.422$^{***}$ & -5.259$^{***}$   \\   & (0.176) & (0.191) & (0.104)   \\  \hline   \\[-1.8ex]  AIC & 13082.630 & 12170.423 & 8030.254   \\  BIC & -191844.071 & -191825.658 & -191914.090   \\  Observations & 368 & 368 & 368   \\ \\  \hline  \hline   \\[-1.8ex]  \textit{Note:} &  \multicolumn{3}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01}  \\  
\end{tabular} 
 \caption{Regression Models for predicting action preferences from misleading and harm judgments (RQ\ref{rq-proxy}). Table only shows the best performing model for each action preference (based on AIC and BIC values)} 
 \label{tab:reg-proxy}
\end{table}



Table \ref{tab:reg-proxy} shows the regression coefficients for the best performing model for each action type. In order to interpret what each model has learned, Figure \ref{fig:rq3:reg_eq} plots the decision boundary of the best fitting model in terms of misleading and harm judgments. That is, for each regression equation, we plot the values for misleading and harm judgments that lead to predicted action preferences of exactly 0.5; articles to the right of the curves are ones where the models predict that more than half of rater would prefer the corresponding action. 

If we were to rely on decision boundary of judgments to make the final action decisions, articles with misleading judgment greater than 3.95 would always be recommended for \textit{inform}. In addition, when the misleading judgment is greater than 4.85, \textit{reduce} would also be recommended as one of the actions. Higher harm scores can lead to the same (or a more stringent) action even when the misleading judgment is lower. For instance, an article with misleading and harm judgments of 4 and 3, respectively, would be recommended for \textit{inform}, while another article with scores of 4 and 5 would be recommended for \textit{reduce} as well. Articles with misleading judgment below 5 would never be recommended for \textit{remove}. When the misleading judgment is higher than 5, the type of action would still depend on the harm judgment. Furthermore, the \textit{reduce} and \textit{remove} decision curves do not intersect the harm-axis, which suggests that harm judgments alone may not be sufficient to recommend an action against an article. This makes sense because most people would not want to remove or reduce distribution of an article containing good information just because the topic was one where misinformation would be harmful. When a topic has a harm score of 7, however, the decision rule would result in placing information labels on all articles. 
Also note that the decision boundary for the \textit{remove} action is a straight line, reflecting that the best fit model did not include an interaction term between the misleading and harm judgments.


% \subsubsection{Comparison between predicted and actual preferences}
Table \ref{tab:rq3:comparison} shows that decisions generated from the output of the misleadingness-harm regression models closely follow the decisions that would be made from taking the majority vote on the preference questions. The Jaccard Index, a popular metric for computing set similarity, shows that the two sets of articles recommended for each action type (one based on prediction, one based on preference) are largely similar. By definition, decisions based on the majority's action preferences produce the fewest disagreements between individual preferences and the decisions. The level of disagreement would be only slightly higher if we used the predictions of the regression models based on aggregate judgments of misleading and harm (Table \ref{tab:rq3:comparison}, right side). 

To understand why, despite some mismatches between the prediction-based decisions and preference-based decisions, the average levels of disagreement are largely similar, consider 
Figure~\ref{fig:rq3:cm}, which shows a confusion matrix-like representation. The vertical dotted line represents a decision-boundary based on expressed preferences of the majority (articles on the right are recommended for action; articles on the left are not) while the horizontal dotted line represents the decision boundary based on predictions from the regression model based on aggregate judgments (articles above the line are recommended for the action; articles below are not). We see that when there is a mismatch between the preference-based decision and judgment-based decision (the upper left and lower right quadrants), the article is usually very close to the decision boundaries, and thus either acting or not acting will both involve around half of raters disagreeing with the choice. 

We also analysed the set of articles that have a prediction-preference mismatch and found no obvious pattern in the topics or other features of the articles (a listing of those articles is in Appendix \ref{app:mismatch}). 


\begin{table}[]
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{} & \multicolumn{2}{c|}{Article set}    & \multicolumn{1}{c|}{\multirow{2}{*}{Jaccard Similarity}} & \multicolumn{2}{c|}{Disagreement (\%age)} \\ \cline{2-3} \cline{5-6} 
                  & Preference-based & Prediction-based & \multicolumn{1}{c|}{}                                    & Preference-based  & Prediction-based \\ \hline
Inform            & 104              & 97 (-8/+1)     & 0.91                                                     & 23.57             & 23.76           \\ \hline
Reduce            & 70               & 70 (-9/+9)       & 0.77                                                     & 21.12             & 21.59             \\ \hline
Remove            & 12               & 17 (-0/+5)       & 0.71                                                      & 11.05            & 11.19             \\ \hline
\end{tabular}
}
\caption{Comparison between decisions based on aggregate preferences and decisions based on the the regression model's output given the aggregate judgments of misleading and harm (Jaccard Index measures similarity between the two set of articles)}
\label{tab:rq3:comparison}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{figures/rq3-cm.png}
    \caption{Comparison between actual preferences and the predicted preferences for each action type; horizontal dotted line represents judgment-based decision boundary, vertical dotted line represents preference-based decision boundary}
    \label{fig:rq3:cm}
\end{figure}


\begin{table}[]
\resizebox{0.4\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
% \multirow{2}{*}{} & \multicolumn{2}{c|}{Level of disapproval (\%age users)}  \\ \cline{2-3} 
\multicolumn{3}{|c|}{Level of Disagreement (\%age users)}          \\ \hline
       & Preference-based & Prediction-based \\ \hline
Inform & 23.28 (SD: 1.72)     & 23.60 (SD: 1.86)                   \\ \hline
Reduce & 21.44 (SD: 1.57)    & 21.89 (SD: 1.57)                  \\ \hline
Remove & 11.7 (SD: 0.98)     & 11.86 (SD: 1.02)                  \\ \hline
\end{tabular}
}
\caption{Prediction performance in terms of the level of disagreement (\%age users) on a held out test set (74 articles) over 10 iterations}
\label{tab:rq3:cv}
\end{table}

\subsubsection{Generalizability of the models}

The cross-validation analysis shows that the results are robust. Table \ref{tab:rq3:cv} shows the prediction performance in terms of the level of disagreement on only the held-out test-set articles, averaged over ten iterations. Even on held-out articles, the level of disagreement with the action selected from the prediction of the regression model from the misinformation and action judgments produces an average level of individual rater disagreement that is only marginally higher than the minimum that could be achieved by always acting on the majority action preference.

% in line with our emphasis on minimizing the overall disagreement associated with the action decisions. Comparing the preference-based outcomes and the judgment-based outcomes of the regression model, the level of disagreement is consistent, suggesting that our models are generalizable and can be used to predict action preferences on completely new articles as well. Additionally, we also report two standard metrics for evaluating predictions -- namely, the F1 score and the Jensen Shannon (JS) distance -- as part of the appendix (see \ref{app:pred}). 


% Table \ref{tab:rq3:cv} shows the prediction performance in terms of the level of disagreement it would create. That is, supposing for held-out items an action were taken whenever the regression model predicted an output of more than 0.5, the table reports the fraction of individual raters who would disagree with that action. The level of disagreement is largely consistent with that obtained using , suggesting that our models are generalizable and can be used to predict action preferences on completely new articles as well.  

% This belongs in discussion; omitting here.
% In summary, we find that relying on users' aggregate judgments about how misleading and harmful content is for predicting their action preferences barely increases the level of individual disagreement with the action decisions. Furthermore, both misleading and harm judgments play a role in the best performing model, and the models we trained are generic enough to predict action preferences on other articles as well. Thus, aggregate action preferences are largely reducible to aggregate judgments of misleadingness and harm, at least when raters are asked to provide misleading and harm judgments prior to reporting their action preferences.


==> _archived__rq.tex <==
\section{Research Questions}
Through our study, we focus on users' preferences for action against misleading news articles and how these preferences may be incorporated into the platforms' moderation process. 
% So far, prior research has shown that the collective judgments of a group of ideologically diverse users aligns very well with the journalists' judgments (often considered as the expert when evaluating misinformation). Furthermore, best results are achieved when users are asked to find and report corroborating evidence before providing their judgments.
% Our study builds on this research and specifically focuses on the users' action preferences against misleading articles.
\rev{Social media} platforms have relied on three different strategies for dealing with misinformation -- inform, reduce, and remove. Inform involves giving users more context on the posts (for instance, adding a misleading label next to the post). Reduce involves reducing the spread of misleading content through algorithmic manipulation (for instance, pushing it lower in a ranked list). Remove involves simply removing the content from the platform. 

In the current setup, these \rev{social media} platforms are largely responsible for deciding when to take each action. For instance, Facebook's guidelines list down the three action types \cite{lyonsHardQuestionsWhat2018} but do not provide any additional information on when each action is taken. Twitter's guidelines\footnote{https://help.twitter.com/en/rules-and-policies/manipulated-media} are somewhat more detailed and present an order of progression -- starting from inform (which is mostly accompanied by reduce) and going up to remove in cases with ``high likelihood of severe harm''. Yet, users' preferences for these different action types are not clear. In particular, how frequently do they want each action to be taken and whether there is a natural order of preference between these actions. Therefore, for our first RQ is as follows:

\emph{\textbf{RQ1:} What is the prevalence and the order of preference between different action types based on the users' aggregate preferences?}
\\
Prior research in political psychology further argues that liberals and conservatives tend to have different moral foundations \cite{grahamLiberalsConservativesRely2009} that may result in different punitive attitudes \cite{silverWhyAreConservatives2017}. Therefore, with regards to taking action against misleading content, conservatives and liberals may have different preferences on how severe an action is and how often it should be taken.

\emph{\textbf{RQ1a:} What are the ideological differences between conservatives and liberals in terms of the prevalence and order of preference between different action types?}
\\
As noted earlier, despite \rev{social media} platforms' emphasis on an objective evaluation of the content, their guidelines for moderating misinformation nevertheless rely on subjective factors like the intention behind the content, and its perceived harmfulness. Furthermore, researchers have generally argued that moderating any content is inherently subjective. As Gillespie further notes, ``no matter where they [platform] draw the line, some users will criticize the platform as too permissive and others as too prudish.'' \cite{gillespieCustodiansInternetPlatforms2018}

For the sake of argument, if misinformation could be moderated objectively, we would expect high-levels of agreement in terms of users preferences for action on each individual article. On the other hand, if it is subjective, then we may observe some cases where the preferences are completely split on whether to take an action or not. Since either of the outcome is not generally acceptable, it would result in high levels of dissent. For our second research question, we investigate the level of dissent associated with our decision outcomes:

% Consequently, a Pew Research survey \cite{noauthor_most_2020} found that only 51\% of the US adults approve of social media platforms taking an action against misleading or inaccurate posts, while only 31\% of them have some confidence in their ability to determine when to take an action. \forlater{maybe mention the line from gillespie about drawing lines...; any other relevant work that talks about this subjectivity angle, from your prior work could also be mentioned here...}

\emph{\textbf{RQ2:} What is the level of dissent associated with the decision outcome that is based on users' aggregate preferences?}
\\
A Pew Research survey in the US found large ideological disparity between Democrats and Republicans in terms of their approval of social media platforms taking any action against misleading content. While 69\% to 72\% of the Democrats expressed their approval, the number dropped to 26\% to 34\% for Republicans \cite{MostAmericansThink2020}. Furthermore, conservatives in the US have repeatedly raised allegations of partisan bias against the platforms \cite{brandtzaegHowJournalistsSocial2017, borelFactCheckingWonUs2017}, arguing that conservative content and sources are overly censored. Having an ideologically diverse set of users should minimize any partisan bias and we explore that by separately computing the dissent level among conservative users and liberal users:

\emph{\textbf{RQ2a:} Is there any disparity between conservatives and liberals in terms of their level of dissent with the decision outcomes?}
\\
When it comes to investigating ideological differences, another important aspect to consider is motivated reasoning. 
% Prior research indicates that users may be susceptible to motivated reasoning,  while evaluating misinformation \cite{kahne_educating_2017}. 
Prior research \cite{allcottSocialMediaFake2017} shows that both conservatives and liberals are more likely to believe in ideologically-aligned misinformation. Subsequently, researchers have also argued that partisan differences in users’ misinformation evaluation are reduced when they are asked to support their judgments with corroborating evidence [under review]. However, this reduction of bias may not directly translate to action preferences, as action against counter-attitudinal content (or a lack of action against pro-attitudinal content) can have direct political gains. 
Since there is no generally acceptable method to account for the ideological bias in each individual article, we use the bias evaluation of the source of that article (as provided by MBFC\footnote{https://mediabiasfactcheck.com/}) as a suitable proxy. Therefore, our third research question is as follows:

\emph{\textbf{RQ3:} Do conservative users want more action than liberal users on articles from pro-liberal sources and vice versa?}
\\
So far, we have emphasized analyzing the decisions based on the users' aggregate preferences. Alternatively, the decisions may also be based on their judgments about how misleading and harmful the content is. Since these judgments are not based on a fixed set of criteria, they may incorporate the subjectivity that is essential for determining users' preferences for different action types. Relying on these judgments adds some value to the moderation process, as the process is no longer specific to a given set of actions. 

We also explore whether one or both of the misleading and harm judgments have a role to play in predicting users' preferences for each action type. Therefore, our next research question is:

\emph{\textbf{RQ4:} Can users' aggregate judgments (misleading or harm) be used to predict their aggregate preferences for different action types?}
